Guiding Energy-based Models via Contrastive Latent Variables

An energy-based model (EBM) is a popular generative framework that offers both explicit density and architectural flexibility, but training them is difficult since it is often unstable and time-consuming. In recent years, various training techniques have been developed, e.g., better divergence measures or stabilization in MCMC sampling, but there often exists a large gap between EBMs and other generative frameworks like GANs in terms of generation quality. In this paper, we propose a novel and effective framework for improving EBMs via contrastive representation learning (CRL). To be specific, we consider representations learned by contrastive methods as the true underlying latent variable. This contrastive latent variable could guide EBMs to understand the data structure better, so it can improve and accelerate EBM training significantly. To enable the joint training of EBM and CRL, we also design a new class of latent-variable EBMs for learning the joint density of data and the contrastive latent variable. Our experimental results demonstrate that our scheme achieves lower FID scores, compared to prior-art EBM methods (e.g., additionally using variational autoencoders or diffusion techniques), even with significantly faster and more memory-efficient training. We also show conditional and compositional generation abilities of our latent-variable EBMs as their additional benefits, even without explicit conditional training. The code is available at https://github.com/hankook/CLEL.

==> table_imagenet32_fid.tex <==
\begin{table}[t]
\centering
\caption{Unconditional MCMC-based generation using EBMs on ImageNet 32$\times$32.}\label{table:imagenet32_fid}
\scalebox{0.9}{%
\begin{tabular}{lc}
\toprule
Method & FID \\ \midrule
IGEBM \citep{du19_igebm}                      & 62.23 \\
Improved CD \citep{du21_improved_cd_ebm}      & 32.48 \\
CF-EBM \citep{zhao2020cfebm}                  & 26.31 \\
\rowcolor{Gray}
{\method}-Base (ours)                              & \textbf{22.16} \\
\bottomrule
\end{tabular}}
\end{table}%


==> table_large_cifar10.tex <==
\begin{table}[t]
\centering
\caption{CIFAR10 Best}
\scalebox{0.9}{%
\begin{tabular}{lccc}
\toprule
Method                 & Params(M) & Time (h) & FID \\
\midrule
Baseline w/o CLEL                      &  6.96 &     & 23.50 \\
+ CLEL               (\textbf{Base})   &  6.96 &  41 & 15.27 \\
+ multi-scale arch.                    & 19.29 &  74 & 12.46 \\
+ CRL with a large batch of 256        & 19.29 &  76 & 10.xx \\
+ more channels (\textbf{Large})       & 30.70 & 133 &  9.23 \\
\midrule
EBM-DRL ($N=2$ blocks)                 &  9.06 &     & 17.34 \\ 
EBM-DRL ($N=8$ blocks)                 & 34.83 & N/A &  9.58 \\ 
\bottomrule
\end{tabular}}
\end{table}
